Online Learning with Unknown Constraints

We consider the problem of online learning where the sequence of actions played by the learner must adhere to an unknown safety constraint at every round. The goal is to minimize regret with respect to the best safe action in hindsight while simultaneously satisfying the safety constraint with high probability on each round. We provide a general meta-algorithm that leverages an online regression oracle to estimate the unknown safety constraint, and converts the predictions of an online learning oracle to predictions that adhere to the unknown safety constraint. On the theoretical side, our algorithm's regret can be bounded by the regret of the online regression and online learning oracles, the eluder dimension of the model class containing the unknown safety constraint, and a novel complexity measure that captures the difficulty of safe learning. We complement our result with an asymptotic lower bound that shows that the aforementioned complexity measure is necessary. When the constraints are linear, we instantiate our result to provide a concrete algorithm with $\sqrt{T}$ regret using a scaling transformation that balances optimistic exploration with pessimistic constraint satisfaction.

==> sec_conclusion.tex <==
\section{Discussion}
We have presented a general algorithm that utilizes online regression and online learning algorithms to produce actions that simultaneously minimize regret while being safe against an unknown constraint with high probability. Furthermore, we introduce a complexity measure that captures the tension between regret minimization and constraint exploration - and show that controlling this complexity measure is necessary for sublinear regret. We conclude with a discussion of potential future directions. First, our algorithms are not efficient beyond simple constraint classes, such as linear functions - we would like to explore computationally efficient algorithms. Our algorithms maintain version spaces over $\F$, which is not tractable without strong assumptions on $\F$. Furthermore, other than when both losses and constraints are linear, our online learning oracle is nonconstructive. Second, we would like to extend the techniques we develop in this paper to richer settings such as reinforcement learning and beyond. 
